Distributed Newton Can Communicate Less and Resist Byzantine Workers

We develop a distributed second order optimization algorithm that is communication-efficient as well as robust against Byzantine failures of the worker machines. We propose COMRADE (COMunication-efficient and Robust Approximate Distributed nEwton), an iterative second order algorithm, where the worker machines communicate only once per iteration with the center machine. This is in sharp contrast with the state-of-the-art distributed second order algorithms like GIANT [34] and DINGO[7], where the worker machines send (functions of) local gradient and Hessian sequentially; thus ending up communicating twice with the center machine per iteration. Moreover, we show that the worker machines can further compress the local information before sending it to the center. In addition, we employ a simple norm based thresholding rule to filter-out the Byzantine worker machines. We establish the linear-quadratic rate of convergence of COMRADE and establish that the communication savings and Byzantine resilience result in only a small statistical error rate for arbitrary convex loss functions. To the best of our knowledge, this is the first work that addresses the issue of Byzantine resilience in second order distributed optimization. Furthermore, we validate our theoretical results with extensive experiments on synthetic and benchmark LIBSVM [5] data-sets and demonstrate convergence guarantees.

==> compress.tex <==
\section{Distributed Newton Can Communicate Even Less}\label{sec:compress}
In Section~\ref{sec:one} we discuss a communication efficient Newton method with only one round of communication per iteration. In this section we further reduce the communication cost by applying a generic class of compressor ($\rho$-approximate compressor) on the update [REF].

\begin{definition}[$\rho$-Approximate Compressor ] \label{def:comp}
An operator $\cQ: \mathbb{R}^d \rightarrow \mathbb{R}^d$ is defined as $\rho$-approximate compressor on a set $S \subset \mathbb{R}^d$ if, $\forall x \in S$,
$
\left\|\cQ(x)-x  \right\|^2 \leq (1-\rho)\left\| x  \right\|^2
$, 
where $\rho \in [0,1]$ is the compression factor. 
\end{definition}

The above definition can be extended for  any randomized operator $\cQ$ satisfying 
$
\mathbb{E}(\left\|\cQ(x)-x  \right\|^2 ) \leq (1-\rho)\left\| x  \right\|^2
$,
for all $\forall x \in S$. The expectation is taken over the randomization of the operator. Notice that $\rho=0$ implies that $\cQ(x)=x$ (no compression).

Each worker machine computes the product of local hessian inverse inverse and local gradient and then apply $\rho$-approximate compressor on this update vector. The $\rho$-approximate compressor encodes the update information of each worker machines in bits and the worker machines communicate these bits to center machine. The center machine aggregates the compressed updates by averaging $\cQ(\hat{\p})= \frac{1}{m}\sum_{i=1}^m \cQ(\hat{\p}_{i,t})$. As the application of the compressor on the update disrupts the update information by a small factor in norm , the aggregated compressed update in the center machine works as a good enough proxy for the exact update while reducing the communication  cost.  In the analysis  we use the following notations: 
\begin{align}
\epsilon_{b}^2 & =(1+\kappa (1-\rho))\epsilon^2 \label{comeps}\\
%\epsilon_{b,\ell}^2 & =(1+\kappa (1-\rho))\epsilon_{\ell}^2\\
\alpha_b^2 & = (1+\kappa (1-\rho))\alpha^2 +\kappa (1-\rho)] \label{comalpha}
\end{align}
where $\epsilon$ is defined in equation~\eqref{eps}, $\kappa$ is the condition number of the Hessian matrix. 

\begin{theorem}\label{thm:byzsmooth}
Let $\mu \in \left[ 1, \frac{n}{d}\right]$ be the coherence of $\bA_t$ . Furthermore, suppose $s \geq  \frac{3\mu d}{\eta^2}\log \frac{md}{\delta}$ for some $\eta,\delta \in (0,1)$. Under Assumption ~\ref{asm:hess}  and with $\cQ$ being the $\rho$-approximate compressor, with probability exceeding $1-\delta$, we obtain
\begin{align*}
  \| \mathbf{\Delta}_{t+1}\| \leq \max \{ \sqrt{\frac{\sigma_{max}(\bH_t)}{\sigma_{min}(\bH_t)}(\frac{\alpha_{b}^2}{1-\alpha_{b}^2})}\| \mathbf{\Delta}_{t}\|, \frac{L}{\sigma_{min}(\bH_t) }\| \mathbf{\Delta}_{t}\|^2  \}+ \frac{ 2\epsilon_{b}}{\sqrt{\sigma_{min}(\bH_t)}},
\end{align*} 
\end{theorem}

\begin{remark}
 In no compression condition, with $\rho=1$ we obtain back the convergence guarantee that of the Theorem~\ref{thm:smooth}.
\end{remark}




==> relt.tex <==
\subsection{Related Work}
\paragraph{Second order Optimization} Second order optimization has received a lot of attention in the recent years in the distributed setting owing to its attractive convergence speed. The fundamentals of second order optimization is laid out in \cite{dane}, and an extension with better convergence rates is presented in \cite{aide}. Recently, in GIANT \cite{giant} algorithm, each worker machine computes an approximate Newton direction in each iteration and the center machine averages them to obtain a \emph{globally improved} approximate Newton direction.  Furthermore, DINGO \cite{dingo} generalizes second order optimization beyond convex functions by extending the Newton-MR \cite{newtonmr} algorithm in a distributed setting. Very recently, \cite{deter} proposes Determinantal averaging to correct the inversion bias of the second order optimization. A slightly different line of work (\cite{wangsketched}, \cite{oversketched}, \cite{newtonsketch}) uses Hessian sketching to solve a large-scale distributed learning problems.

%\begin{itemize}
%\item DANE\cite{dane}:  It is a stochastic optimization method where in each iteration the worker machine performs a local optimization and the master aggregates the model parameter by taking average of the model parameter of each worker machines.
%
%\item AIDE \cite{aide} : The author develops  a robust version of DANE \cite{dane} where each worker outputs an approximate  solution to the local problem. Also an  accelerated version of the algorithm is presented in the paper.
%
%\item GIANT \cite{giant}: Each local user computes a approximate Newton direction in each iteration and the master performs an averaging method to obtain a \emph{globally improved } approximate Newton direction.
%
%\item Determinantal averaging: \cite{deter}: The author proposes a \emph{determinantal averaging} to correct the inversion bias of the second order optimization.
%
%\item Newton-MR \cite{newtonmr}: The authors generalizes the \emph{Newton-CG} method beyond the strongly convex assumption. 
%
%
%\item DINGO \cite{dingo}: This is a distributed variant of the Newton-MR\cite{newtonmr} algorithm where the gradient's norm is used as a surrogate function for the empirical minimization objective.
%
%\item DiSCO \cite{disco}: The author  design algorithm for optimization with regularized empirical loss function and use the self-concordance property of the loss to weaken the dependence of the condition number in the convergence rate of the Newton algorithm.
%
%\item \cite{wangsketched}: The authors studies the optimization and statistical impact of the Hessian sketch in Matrix ridge regression.
%
%\item Over-sketched Newton \cite{oversketched}: the author studies a randomized Hessian-based optimization algorithm to solve large-scale convex optimization problems in serverless systems. 
%  
%\item Newton Sketch \cite{newtonsketch}: The author proposes a randomized second order method where the approximate Newton step is computed using projected or sub-sampled Hessian.
%\end{itemize}


\paragraph{Byzantine Robust Optimization:} In the seminal work of \cite{feng},  a generic framework of one shot median based robust learning has been proposed and analyzed in the distributed setting.  The issue of Byzantine failure is tackled by grouping the servers in batches and computing the median of batched servers in
\cite{chen} (the median of means algorithm). Later in \cite{dong,dong1}, co-ordinate wise median, trimmed mean and iterative filtering based algorithm have been proposed and
optimal statistical error rate is obtained. Also,  \cite{mhamdi2018hidden,Damaskinos} consider adversaries may steer convergence to bad local minimizers for non-convex optimization problems.

